NeuJeans: Private Neural Network Inference with Joint Optimization of Convolution and FHE Bootstrapping

Fully homomorphic encryption (FHE) is a promising cryptographic primitive for realizing private neural network inference (PI) services by allowing a client to fully offload the inference task to a cloud server while keeping the client data oblivious to the server. This work proposes NeuJeans, an FHE-based solution for the PI of deep convolutional neural networks (CNNs). NeuJeans tackles the critical problem of the enormous computational cost for the FHE evaluation of CNNs. We introduce a novel encoding method called Coefficients-in-Slot (CinS) encoding, which enables multiple convolutions in one HE multiplication without costly slot permutations. We further observe that CinS encoding is obtained by conducting the first several steps of the Discrete Fourier Transform (DFT) on a ciphertext in conventional Slot encoding. This property enables us to save the conversion between CinS and Slot encodings as bootstrapping a ciphertext starts with DFT. Exploiting this, we devise optimized execution flows for various two-dimensional convolution (conv2d) operations and apply them to end-to-end CNN implementations. NeuJeans accelerates the performance of conv2d-activation sequences by up to 5.68 times compared to state-of-the-art FHE-based PI work and performs the PI of a CNN at the scale of ImageNet within a mere few seconds.

==> Backup/3_method_old.tex <==
\section{Leaner Convolution in the Frequency Domain}\label{sec:algorithm}

\begin{figure*}[t]
\centering
\includegraphics[width=.7\textwidth]{fig/dft-conv.pdf}
\label{fig:dft-conv}
\caption{High-level overview of our convolution method.}
% Server preprocesses weight kernels by performing zero-padding, $DFT_l$ ($\mathsf{S_{l\leftarrow{0}}}$), and fusing with StoC posterior ($\mathsf{S_{\frac{N}{2}\leftarrow{l}}}$). Client evalutes $DFT_l$ on each image and sends encrypted images to the server. Server performs block matrix-vector multiplication which results in Fourier transformed convolution results.
\end{figure*}

{\jyp{*JYP: process/preprocess, such word choice might be seen as negative aspects of our approach invoking some additional server offline/client online computation cost. Should we keep them?}}

Given input ciphertext processed by the client, and the kernels preprocessed by the server, the CNN convolution layer can be efficiently evaluated. Specifically, if $B$ input feature maps fit into one ciphertext, a convolution layer with $B$ input channels and $B$ output channels can be evaluated with $\Theta(2\sqrt{B})$ homomorphic rotations. The algorithm can be generalized to evaluate a $C_{in}$ input channels and $C_{out}$ output channels with $\Theta(2\sqrt{\frac{C_{in}C_{out}}{B}})$ homomorphic rotations.



\subsection{Input Processing and Kernel Preprocessing}\label{sec:preprocess}
We assume the input ciphertext encrypts a vector which is acquired by the following steps: (1)~zero pad each input feature map, (2)~flatten in row-major order, (3)~apply DFT to each flattened vector, (4)~concatenate.

The feature maps are zero padded such that the total spatial size becomes a power of two. The size of the padded feature map is $M={\iwidth}\times {\iwidth}  = 2^{\lceil \log_2{{\iwidth}_0} \rceil} \times 2^{\lceil \log_2{{\iwidth}_0} \rceil}$. Then, $B=(N/2)/M$ padded feature maps fit in a single message. Each kernel is also padded such that a padded kernel occupies the same space as a padded feature map. That is, the size of each padded kernel is also ${\iwidth}\times {\iwidth}$, where ${\iwidth}^2-{{\kwidth}}^2$ of the ${\iwidth}^2$ elements are zeros. Again, $B$ padded kernels fit in a single message. Details about the zero padding will be later discussed in Section~\ref{sec:zeropad}.

The n-th channel of input feature map $I_n$ is zero padded and flattened in row-major order into a vector $\mathbf{i_{n}}$. The kernel $K_{m,n}$ is similarly zero padded and flattened into a vector $\mathbf{k_{m,n}}$. However, when flattening the kernel in row-major order, the order is reversed. This is because the CNN convolution is identical to traditional convolution with flipped kernels.

Next, DFT is applied to each of the flattened feature maps and kernels. Finally, the feature maps for different input channels are concatenated sequentially into $\mathbf{x_i^{(\ell)}}$. If $C_{in}>B$, the first $B$ channels are packed into $\mathbf{x_0^{(\ell)}}$, the next $B$ channels into $\mathbf{x_1^{(\ell)}}$ and so on. The kernels corresponding to different input channels $\{c_{k,0}, c_{k,1}, ..., c_{k,B-1}\} \subseteq [C_{in}]$ and different output channels $\{{c'}_{k,0}, {c'}_{k,1}, ...,{c'}_{k,B-1}\} \subseteq [C_{out}]$ are concatenated into a vector $\mathbf{w_k^{(\ell)}}$. We use both $\mathcal{F(\cdot)}$ and $\hat{}$ to denote 1D DFT. The meaning of the superscript $\ell$ will be explained in the later sections.

\small
\begin{equation}\label{eq:localDFT}
\mathbf{x_0^{(\ell)}} = \begin{bmatrix}
               \mathcal{F}(\mathbf{{I}_{{1}}}) \\
               \mathcal{F}(\mathbf{{I}_{{2}}}) \\
               \vdots \\
               \mathcal{F}(\mathbf{{I}_{{B}}})
               \end{bmatrix}
            = \begin{bmatrix}
               \mathbf{\hat{I}_{{1}}} \\
               \mathbf{\hat{I}_{{2}}} \\
               \vdots \\
               \mathbf{\hat{I}_{{B}}}
               \end{bmatrix}
,
\mathbf{w_k^{(\ell)}} 
               % = \begin{bmatrix}
               % \mathcal{F}(\mathbf{{K}^{{c'}_{k,0}, c_{k,0}}}) \\
               % \mathcal{F}(\mathbf{{K}^{{c'}_{k,1}, c_{k,1}}}) \\
               % \vdots \\
               % \mathcal{F}(\mathbf{{K}^{{c'}_{k,B-1}, c_{k,B-1}}})
               % \end{bmatrix}
               = \begin{bmatrix}
               \mathbf{\hat{k}_{{c'}_{k,1}, c_{k,1}}} \\
               \mathbf{\hat{k}_{{c'}_{k,2}, c_{k,2}}} \\
               \vdots \\
               \mathbf{\hat{k}_{{c'}_{k,B}, c_{k,B}}}
               \end{bmatrix}
\end{equation}
\normalsize

Then, the client will encode, encrypt, and send the results as \ct{$\mathbf{x_0^{(\ell)}}$}. The server should have encoded and saved the results as \pt{$\mathbf{w_k^{(\ell)}}$} before starting the service.

\subsection{For a Single Ciphertext}

Assume the simple case where $C_{in}=C_{out}=B$ . Then, $\{c_{k,0}, c_{k,1}, ..., c_{k,B-1}\} = [C_{in}]$, and $\{{c'}_{k,0}, {c'}_{k,1}, ..., {c'}_{k,B-1}\} = [C_{out}]$ for $k\in[0,B)$. Now we will discuss how to choose the order of these channels during the concatenation step of Section~\ref{sec:preprocess}, and how to evaluate frequency domain convolution.

First, the elementwise multiplication of the vectors $\mathbf{\hat{I}_n}$, $\mathbf{\hat{K}_{m,n}}$ evaluates the SISO convolution in the frequency domain. Although we applied 1D DFT, and thus the convolution is 1D, the zero padding makes the result almost identical to the result of SISO convolution. Specifically, $\mathbf{\hat{K}_{i, j}} \odot \mathbf{\hat{I}_j}=\mathcal{F}(\mathbf{{K}_{i, j}}\ast\mathbf{{I}_j}) = \mathcal{F}(\mathbf{{O'}_i}) = \mathbf{\hat{O'}_i}$, where $\mathbf{{O'}_i}$ is $O_i$ which got processed in the same way as $I_j$, but padded with garbage values instead of zeros. This will be later discussed in Section~\ref{sec:zeropad}. 

Therefore, a single elementwise multiplication of the two vectors $\mathbf{w_{{c'}_i}^{(\ell)}}$, $\mathbf{x_0^{(\ell)}}$ lead to the parallel evaluation of $B$ SISO convolutions.
%As in the previous sections, we will omit the conversion of $<<$ and $\odot$ into their corresponding homomorphic operations \textrm{HRot} and \textrm{PMult}.

\small
\begin{equation*}
\mathbf{w_{{c'}_i}^{(\ell)}}\odot\mathbf{x_0^{(\ell)}}
               \!=\! \begin{bmatrix}
               \mathbf{\hat{k}_{{c'}_{i}, c_{0}}} \odot\mathbf{\hat{I}_1}\\
               \mathbf{\hat{k}_{{c'}_{i}, c_{1}}} \odot\mathbf{\hat{I}_2}\\
               \vdots \\
               \mathbf{\hat{k}_{{c'}_{i}, c_{B-1}}} \odot\mathbf{\hat{I}_B}
               \end{bmatrix}
                \!=\! \begin{bmatrix}
               \mathcal{F}(\mathbf{{k}_{{c'}_{i}, c_{0}}}\ast\mathbf{{I}_1}) \\
               \mathcal{F}(\mathbf{{k}_{{c'}_{i}, c_{1}}}\ast\mathbf{{I}_2)} \\
               \vdots \\
               \mathcal{F}(\mathbf{{k}_{{c'}_{i}, c_{B-1}}}\ast\mathbf{{I}_B})
               \end{bmatrix}
\end{equation*}
\normalsize

Also, if the Fourier transformed vectors weren't concatenated, the frequency domain convolution can be evaluated as the following:

\[\mathbf{\hat{O'}_i} = \sum_{j=1}^{B}\mathbf{\hat{K}_{i, j}}\odot\mathbf{\hat{I}_j}\]

Notice how the index patterns are identical to a matrix-vector multiplication: e.g. $\mathbf{y}=\mathsf{A}\mathbf{x}$, $(\mathbf{y})_i = \sum_{j}\mathsf{A}_{ij}(\mathbf{x})_j$. The only difference with a normal matrix-vector multiplication, is that vectors are in the place of scalar values, and elementwise multiplication is in the place of scalar multiplcation. Thus, the frequency domain convolution can be viewed as a matrix-vector multiplication with each element being an equal sized vector, where elementwise multiplication is used as multiplication. Now consider the following block matrix~$\mathsf{W}_l$:

\small
\begin{equation*}
\mathsf{W}_l
\!=\! \begin{bmatrix}
diag(\mathbf{\hat{k}_{1, 1}}) & diag(\mathbf{\hat{k}_{1, 2}}) & \dots & diag(\mathbf{\hat{k}_{1, B}}) \\
diag(\mathbf{\hat{k}_{2, 1}}) & diag(\mathbf{\hat{k}_{2, 2}}) & \dots & diag(\mathbf{\hat{k}_{2, B}}) \\
\vdots & \vdots & \ddots & \vdots \\
diag(\mathbf{\hat{k}_{B, 1}}) & diag(\mathbf{\hat{k}_{B, 2}}) & \dots & diag(\mathbf{\hat{k}_{B, B}})

\end{bmatrix}
\end{equation*}
\normalsize

Here, $diag(\mathbf{\hat{k}_{i, j}})$ is a diagonal matrix with $\mathbf{\hat{k}_{i, j}}$ as the diagonal. Since block matrices and block vectors with the same block size act as each block is an element and $diag(\mathbf{\hat{K}^{i, j}})\mathbf{\hat{I}^j} = \mathbf{\hat{K}^{i, j}}\odot\mathbf{\hat{I}^j}$, the following holds.

\begin{equation*}
\mathsf{W}_l\mathbf{x^0_l}
= \mathsf{W}_l\begin{bmatrix}
               \mathbf{\hat{I}_{1}} \\
               \mathbf{\hat{I}_{2}} \\
               \vdots \\
               \mathbf{\hat{I}^{B}}
               \end{bmatrix}
= \begin{bmatrix}
               \mathbf{\hat{O'}_{1}} \\
               \mathbf{\hat{O'}_{2}} \\
               \vdots \\
               \mathbf{\hat{O'}_{B}}
               \end{bmatrix}
\end{equation*}

Therefore, frequency domain convolution is nothing more than a single matrix-vector multiplication. In addition, the matrix $\mathsf{W}_l$ has a very special shape. It is a block matrix with all blocks being a diagonal matrix of equal size $M\times M$. If we change the point of view, $\mathsf{W}_l$ is a $N/2\times N/2$ matrix with $B$ evenly spaced nonzero diagonals. The space between the nonzero diagonals is $M$, the size of the padded feature map. We will call matrices of this shape as \emph{striped matrices} or \emph{striped matrices with spacing M}. 

As in Equation~(\ref{eq:matvecmul}), the matrix-vector multiplication with $\mathsf{W}_l$ can be expressed as the following.

\begin{equation*}
\mathsf{W}_l\mathbf{x_0^{(\ell)}} = \sum_{k=1}^{B}diag(\mathsf{W}_l, Mk)\odot(\mathbf{x_0^{(\ell)}}<<Mk)
\end{equation*}

Therefore, the matrix-vector multiplication can be efficiently calculated if $\mathbf{{w}^{(\ell)}_{k}} = diag(\mathsf{W}_l, Mk)$. Then ${c'}_{k,b}$ and ${c}_{k,b}$ for $b\in[0,B)$ are the output and input channel corresponding to the $b$th block in the $k$th nonzero diagonal of $\mathsf{W}_l$. This is similar to the diagonal matrix packing in Section~\ref{sec:background:diagonal pack}, but we are packing the kernels diagonally, from a matrix of kernels, rather than the scalar values (Figure~\ref{fig:diagKernels}). This diagonal packing of kernels is similar to the method used in \cite{juvekar_2018_gazelle}. However, the DFT removes the need for rotations when evaluating SISO convolutions.

From \emph{Remark}~\ref{remark:bsgs}, this matrix-vector multiplication can be evaluated with $\Theta(2\sqrt{B})$ homomorphic rotations. If $\sqrt{B}$ is an integer, it can be evaluated with $2\sqrt{B}-2$ rotations.

Also note that the product of striped matrices with the same spacing will also be a striped matrix with the same spacing. A striped matrix with spacing $M$ is equal to a block matrix with all blocks being a $M\times M$ diagonal matrix. Since when multiplying block matrices we can treat each block as an element, and the sum and product of diagonal matrices is also a diagonal matrix, the product of striped matrices with the same spacing will also be a block matrix with all blocks being a diagonal matrix. This property will be used later in the paper.

\begin{figure}
\centering
\includegraphics[width=.99\columnwidth]{fig/temp_diagonalKernels.jpeg}
\label{fig:diagKernels}
\caption{ The kernels are packed diagonally. This is just the diagonal matrix packing in Section~\ref{sec:background:diagonal pack} applied to a block matrix.}
\end{figure}

\begin{remarkk}
Frequency domain convolution is a matrix-vector multiplication with a striped matrix with spacing $M$. Where $M$ is the size of the padded feature map.
%This costs $\Theta(2\sqrt{B})$ homomorphic rotations using BSGS, where $B$ is the number of nonzero diagonals in the striped matrix.
\end{remarkk}

\begin{remarkk}
The product of striped matrices with the same spacing is also a striped matrix with the same spacing. 
\end{remarkk}


\subsection{For Multiple Ciphertexts}
As in the previous section, we also use diagonal packing from the matrix of kernels. However, since only $B < C_{in}, C_{out}$ input feature maps / kernels fit into a single plaintext / ciphertext, we view the matrix of kernels as a block matrix. Each block will have $B\times B$ kernels. We will also view the input vector as a block vector, where each block is a vector of $B$ feature maps. We can evaluate the large matrix-vector multiplication while treating these blocks as elements, and the multiplication between these elements as the matrix-vector multiplication in the previous section.

\subsection{Zero Padding}\label{sec:zeropad}

%\section{Joint Evaluation with Bootstrapping}
\section{Fusing Domain Switch with Bootstrapping}
%-------------------------------------------------------------------------------
%We will set $M = {\iwidth}^2$, $B=(N/2)/M$, and $l=\log_{2}M=\log_2{{\iwidth}^2}.
%The bootstrapping process consists of three operations: Coefficient To Slot(CtoS), Modular Evaluation(ModEval), Slot To Coefficient(StoC). StoC(and also CtoS) is a linear operation that computes a variant of discrete Fourier transform(DFT).
CtoS and StoC can be efficiently computed with FHE by factorizing the DFT matrix, generalizing the Cooley-Tukey algorithm~\cite{chen_2019_improved}.
Computation using the factorization is equivalent to applying DFT independently to fixed length partitions of a ciphertext, which is similar to how multi-dimensional DFTs are performed.
%This sequential computation of this factorization is essentially applying DFT independently to fixed length partitions of a ciphertext.

This \emph{localDFT} can be used for domain switching multiple images simultaneously for the evaluation of convolution in the frequency domain. Specifically, it can be used to generate a ciphertext encrypting the vector $\mathbf{x_0^{(\ell)}}$ in Equation~(\ref{eq:localDFT}).

The size of the feature maps may vary per CNN layers, thus we need to freely be able to choose the length in which DFT is independently applied. By choosing how to slice StoC-by choosing the factorization of the DFT matrix-we can choose this length. 
% Setting the length as the size of an image lends the SISO convolution with only a single ciphertext-plaintext multiplication. Multiple simultaneous SISO convolutions are possible if multiple images can fit inside a single ciphertext.

% The previous method\cite{kim2023optimized} only utilized the full StoC process, which evaluated DFT over the entire ciphertext. This \emph{globalDFT} is used to perform convolution with elementwise multiplication. However to use globalDFT, kernels from different output channels must be packed into different ciphertexts. If not, the global convolution following globalDFT will interleave the parameters from different output channels, which should not happen in CNN layers. Thus the convolution for each output channels needed to be calculated separately, then packed for the next layer using a rotation intensive method\cite{chen2021efficient}.

% \temp{LocalDFT essentially applies DFT to elements of the consecutive, equally sized partition of a message vector. For convenience, we will call these elements \emph{blocks}. A message vector of size $N/2$ can be viewed as a concatenation of $B$ blocks of size $M=(N/2)/B$.}

\subsection{StoC Anterior is LocalDFT}
In the CKKS scheme, for a ciphertext \ct{$\mathbf{x_0}$}, where the message $\mathbf{x_0} \in \mathbb{C}^{N/2}$ is slot encoded, StoC evaluates the matrix-vector multiplication of the DFT matrix $\mathsf{S}$ and $\mathbf{x_0}$ homomorphically. Bit-reversal is also fused into $\mathsf{S}$ in order to apply the Cooley-Tukey algorithm. Using the algorithm, $\mathsf{S}$ can be factorized into $\log_{2} {N/2}$ matrices.

\[\mathsf{S}=\mathsf{S}_{\log_{2} {N/2}}\mathsf{S}_{\log_{2} {N/2} - 1}\cdots\mathsf{S}_3\mathsf{S}_2\mathsf{S}_1\]

These matrices can be collapsed freely to optimize the tradeoff between level consumption and the number of rotations~\cite{chen_2019_improved}. The product of matrices $\mathsf{S_f}\mathsf{S_{f-1}}\cdots\mathsf{S_{i+2}}\mathsf{S_{i+1}}$ will be denoted as $\mathsf{S}_{{f}\leftarrow{i}}$, so that $\mathsf{S}=\mathsf{S}_{\log_{2}{N/2}\leftarrow{0}}$. Then, $\mathbf{x_l}=\mathsf{S}_{l\leftarrow{0}}\mathbf{x_0}$ becomes the following.

\[(\mathbf{x_l})_{Mb+k}=\sum_{m=0}^{M-1}(\mathbf{x_0})_{{Mb+\sigma_{\log_{2}M}(m)}}(\zeta_k^B)^m\]

Where $M=2^{l}$ denotes the size of a single 'block', and $B=(N/2)/{2^l}=(N/2)/M$ is the number of blocks inside a single slot encoded message. $m$ and $k$ are the internal indices for each block ($0\le{m,k}<M$), and $b$ is the block index ($0\le{b}<B$). $\sigma_{\log_{2}M}$ indicates bit reversal for $\log_{2}M$ bits. Thus when DFT is applied to each block, the elements are indexed in bit-reversed order (Figure~\ref{fig:localDftIndexing}). Also notice that this equation becomes a full expression of $\mathsf{S}$ when $l=log_2{N/2}$.

% \begin{figure}
% \centering
% \includegraphics[width=.99\columnwidth]{fig/temp_localDftIndexing.jpeg}
% \label{fig:localDftIndexing}
% \caption{The anterior of StoC applies DFT locally to each block of the message.}
% \end{figure}

The bit reversal of each block that happens during localDFT can be canceled out by encoding a message with each blocks already bit reversed. By setting $(\mathbf{x_0})_{{Mb+\sigma_{\log_{2}M}(m)}} = \mathbf{X}_{Mb+m}= \mathbf{X}_{b,m}$ (the $m$th element of the $b$th block), localDFT with no bit reversal can be applied to the vector $\mathbf{X} \in \mathbb{C}^{N/2}$.

\[(\mathbf{x_l})_{Mb+k}=\sum_{m=0}^{M-1}\mathbf{X}_{Mb+m}(\zeta_k^B)^m=\sum_{m=0}^{M-1}\mathbf{X}_{b,m}(\zeta_k^B)^m\]

Homomorphically evaluating elementwise multiplication with another message after localDFT, will yield the 1D convolutions of the corresponding blocks of each message. Note that localDFT(the multiplication with $\mathsf{S_{l\leftarrow{0}}}$) can be directly applied to message vectors before encoding nor encrypting, as a type of preprocessing. Blockwise 1D convolution with a vector $\mathbf{Y} \in \mathbb{C}^{N/2}$ of fixed values can be obtained by preprocessing and encoding $\mathbf{Y}$ into a plaintext \pt{$\mathbf{y_l}$} $=$ \pt{$\sum_{m=0}^{M-1}\mathbf{Y}_{Mb+m}(\zeta_k^B)^m$} $=$ \pt{$\sum_{m=0}^{M-1}\mathbf{Y}_{b,m}(\zeta_k^B)^m$}, then evaluating PMult.

\[\textrm{PMult}([\langle\mathbf{x_l}\rangle], \langle\mathbf{y_l}\rangle) = [\langle\sum_{m=0}^{M-1} (\sum_{t=0}^{M-1}\mathbf{X}_{b,t}\mathbf{Y}_{b, m-t})(\zeta_k^B)^m\rangle]\]
\[\mathbf{Y}_{b, m-t} = \begin{cases} 
                    \mathbf{Y}_{b, m-t} & m-t \ge 0 \\
                    j\mathbf{Y}_{b, M+m-t} & m-t < 0 \\
                        \end{cases}\]

During this elementwise multiplication, the exponent of the twiddle factor $\zeta_k^B$ becomes larger than the block size $M$ for some terms, causing them to \emph{wrap around}. $(\zeta_k^B)^M=e^{2\pi j BM5^k/ 2N}=(e^{\pi j/2})^{5^k}=j^{5^k}=j$ is multiplied to the wrap around terms instead of one. Hence $j$ is multiplied to $\mathbf{Y}_{b, M+m-t}$ when $m-t < 0$. In this special convolution, a value must wrap around four times to return to its original state. $-j$ can be multiplied to certain elements of $\mathbf{Y}$ to cancel out this effect. In other words, the \emph{j-cyclic convolution} is evaluated for elementwise multiplications after StoC anterior.
%. and use the symbol $\hat{\ast}$.

\begin{remarkk}
The StoC anterior $\mathsf{S}_{{\ell}\leftarrow{0}}$ locally applies bit-reverse permutation and DFT to blocks of size $2^\ell$.
\end{remarkk}

\subsection{LocalIDFT using StoC and CtoS}
In Section~\ref{sec:algorithm}, we acquired the output feature maps in the frequency domain. In order to evaluate the nonlinear activation functions, we must apply IDFT locally. It turns out that the composition of StoC posterior and CtoS becomes the LocalIDFT.

From the previous section, we know that the StoC anterior $\mathsf{S}_{{\ell}\leftarrow{0}}$ is localDFT. We also know that the CtoS operation is essentially multiplying $\mathsf{S}^{-1}=(\mathsf{S}_{{N/2}\leftarrow{\ell}}\mathsf{S}_{{\ell}\leftarrow{0}})^{-1}=\mathsf{S}_{{\ell}\leftarrow{0}}^{-1}\mathsf{S}_{{N/2}\leftarrow{\ell}}^{-1}$. Thus the composite evaluation of StoC posterior and CtoS becomes localIDFT: $\mathsf{S}^{-1}\mathsf{S}_{{N/2}\leftarrow{\ell}}=\mathsf{S}_{{\ell}\leftarrow{0}}^{-1}$.

\subsection{Putting Things Together}
Multiple layers of convolution can be evaluated in the following method. For simplicity, we assume the padded image size is fixed to $M$ where $M\times B = N/2$ and there are $B$ input channels and $B$ output channels. $\mathbf{x_i^{(0)}}$ is a vector where the feature maps from the $i$th convolution are concatenated.

(1) The client concatenates the flattens images into $\mathbf{x_0^{(0)}}$ and applies the StoC anterior before encryption. The vector is then encrypted and sent to the server. (message = $\mathsf{S}_{{\ell}\leftarrow{0}}\mathbf{x_0^{(0)}}$)

(2) The server evaluates convolution in the frequency domain using preprocessed kernels. (message = $\mathsf{W^{(\ell)}}\mathsf{S}_{{\ell}\leftarrow{0}}\mathbf{x_0^{(0)}}=\mathsf{S}_{{\ell}\leftarrow{0}}\mathbf{x_1^{(0)}}$)

(3) The rest of the bootstrapping (StoC posterior, CtoS, ModEval) is computed. This evaluates localIDFT. (message = $\mathbf{x_1^{(0)}}$)

(4) 


\begin{figure}
\centering
\includegraphics[width=.99\columnwidth]{fig/fig_packLocalDFT_mutichannel.png}
\label{fig:packLocalDFT}
\caption{ Multiple SISO convolutions are evaluated via a single elementwise multiplication in the frequency domain. StoC anterior is a combination of 1D DFT and bit-reverse permutation. To cancel out bit-reverse permutation, all feature maps and kernels are bit-reverse permuted. }
\end{figure}

% \subsection{Applying LocalDFT to CNN}
% Multiplying $\mathsf{S}_{l\leftarrow{0}}$ to these vectors on the left(i.e. applying localDFT) will apply a variant of 1D DFT to each of the flattened and concatenated feature maps/kernels. A following elementwise multiplication between $\mathbf{x_l}=\mathsf{S}_{l\leftarrow{0}}\mathbf{x_0}$ and $\mathbf{y_l}=\mathsf{S}_{l\leftarrow{0}}\mathbf{y_0}$ will evaluate the $j$-cyclic convolution for each block, in the frequency domain. The zero paddings allow accurate evaluation of SISO convolutions via the $j$-cyclic convolutions.

% \temp{...}

% An example of this process is shown in Figure~\ref{fig:packLocalDFT}. An $1\times 1$ kernel is zero padded into $2\times 2 = W \times W$ space and $p$ is set to $0$. 



%=\sum_{i=0}^{W-1}\sum_{j=0}^{W-1}\mathbf{{I}^{c_{b}}}_{{\iwidth}\cdot i + j}(\zeta_k^B)^{{\iwidth}\cdot i + j}\end{aligned}\]


%\subsubsection{Blockwise Baby-Step Giant-Step}





% \subsubsection{BSGS Tradeoff with Multiple Ciphertexts}
% The tradeoff between baby-steps and giant-steps differ when all feature maps of a layer do not fit into a single ciphertext. This is because the computation pattern allows us to further reduce the number of rotations.

% When $C_n$ feature maps fit in a single ciphertext, we divide the kernel matrix into $C_{out}/C_n \times C_{in}/C_n$ blocks. Then, we can 

% Such division of the kernel matrix is also used in ~\cite{juvekar_2018_gazelle}. However, there is no need for the SISO rotations nor the SISO packing, which essentially disassembles the convolution between a single layer kernel of size $k\times k$ and a single feature map, into $k^2$ multiplications with $k^2$ plaintexts, and $k^2$ ciphertext rotations. Even with the usage of the BSGS algorithm, this requires $k$ times more ciphertext rotations, and $k^2$ times more plaintext compared to NeuJeans.

\section{Fusion with StoC Posterior}
%-------------------------------------------------------------------------------
% \subsection{Striped Matrices}



\subsection{StoC Posterior}

\begin{remarkk}
Both the StoC posterior matrix and the frequency domain convolution matrix are striped matrices. These two striped matrices have the same spacing if the StoC anterior was used for localDFT.
\end{remarkk}

+level scheduling

Collapsing the StoC posterior matrices may increase the number of rotations needed for the operation. However, the overall number of rotations decrease, since the rotations for the collapsed StoC are those that were already necessary for the convolution operation. Thus when convolution layers are computed after the localDft, StoC posterior can be jointly evaluated for free.

one less level spent, making StoC cheaper

\begin{figure}
\centering
\includegraphics[width=.99\columnwidth]{fig/temp_StoCPosteriorAndConvFusion.jpeg}
\label{fig:StoCPosteriorFusion}
\caption{StoC Posterior and the convolutional layer can be fused with no cost. The memory size of parameters and the computational complexity after fusion is identical to those of just the convolutional layer. The LocalDft applied in StoC Anterior simplifies the convolution into multiplications, allowing the free piggyback of StoC Posterior.}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=.99\columnwidth]{fig/temp_lowLevelDueToFusion.jpeg}
\label{fig:lowLevelDueToFusion}
\caption{Level scheduling of NeuJeans and the previous scheme~\cite{kim2023optimized}.}
\end{figure}

\subsection{General Fusion with Bootstrapping}


%\section{Accurate ReLU Evaluation}

\section{Other Techniques}
\subsection{Scheduling of Strided Convolution}
Strided Conv2D can be rewritten as several unit-strided Conv2D. Downsampling layers reduce the image size resulting in sparsely encoded ciphertexts, which leads to slot underutilization. Unlike unencrypted data, a sparse ciphertext can't be reorganized to a dense ciphertext by simply changing memory addresses. Such densify operation requires multiplications with mask, a plaintext which holds 0 or 1 in its slot, and heavy rotations. However, as the strided Conv2D necessitates to bootstrap ciphertexts before the densify operation, the number of bootstrapping expands severely. 

In contrast, our downsampling algorithms are free of such bootstrapping expansion. Our algorithmic shift enables densify operation to be placed in front, thereby bootstrapping on dense ciphertexts. This simple modification effectively reduces the number of bootstrapping by $s\times s$-fold.  
We present our algorithm in Figure~\ref{}.
When stride is $s$, we first divide an input image I and a kernel K to $s^2$ fragments by 


If such reduction happens after bootstrapping, the number of bootstrapping for the layer will quadruple/double. This was not a significant problem in ~\cite{kim_2023_optcnn} because the method was only used for latter parts of ResNet18, where feature maps can fit into a small number of ciphertexts and strided convolutions appear once per four convolution layers. However, if the size reduction due to the initial strided convolution is scheduled after boostrapping, this may more than double the total number of bootstrapping. An Imagenet input image is initially $3\times224\times224$

\begin{figure}
\centering
\includegraphics[width=.99\columnwidth]{fig/temp_StridedConvScheduling.jpeg}
\label{fig:jobScheduling}
\caption{By rearranging the feature map such that strided convolutions become the sum of convolutions with smaller size, the number of bootstrapping needed for the layer is halved.}
\end{figure}

BSGS can be used for sparse-to dense gathering, although it was not used in [Optimized], we decided to implement it to both when evaluating

% \begin{figure}
% \begin{center}
% \includegraphics[width=.49\textwidth]{fig/temp_rearrangementForStridedConv.jpeg}
% \end{center}
% \caption{\label{fig:stridedConv} \temp{JJU: this figure is the least needed. just describing the algorithm would be enough. but still, 'I' would take ages to understand this without this figure if this was the first time seeing this. How kind do we have to be?}}
% \end{figure}

\subsection{Depthwise Convolution and Average Pooling}

In [Optimized] it is impossible to select blocks of the ciphertext to be convoluted.



%\subsection{Max Pooling}
\subsection{Network Retraining}

\subsection{Utilizing Complex Message}
\temp{this should go somewhere else}
%-------------------------------------------------------------------------------

% \temp{TEMP WRITING: SYMBOLS!}

% $M$ : size of a single block when LocalDFT is applied

% $m$ : index for elements inside a LocalDFT block

% $B$ : the number of blocks inside a vector when LocalDFT is applied ($M\times B = N/2$)

% $b$ : index for blocks inside a vector

% $C_{in}$ : total number of input channels

% $c_{in}$ : an index for input channel

% $C_{out}$ : total number of output channels

% $c_{out}$ : an index for output channel

% $w$ : the width of a zero padded feature map / zero padded kernel

% $w_0$ : the width of a feature map

% $f$ : the width of a kernel

% $\mathbf{x}$, $\mathbf{y}$ : general vector

% $\mathbf{x^i}$, $\mathbf{y^i}$ : ith vector

% $\mathbf{x_l}$, $\mathbf{y_l}$ : vectors with $2^l$ size localDFT applied

% $\mathbf{W^i}$ : ith diagonal-packed weight vector

% $\mathbf{K^{c_{out}, c_{in}}}$ : Kernel for a certain input/output channel: 

% $\mathbf{I^{c_{in}}}$ : Feature map for a certain input channel

% $\mathsf{I}$ : identity matrix

% $\mathsf{S}$ : slot to coefficient matrix

% $\mathsf{P}$ : bit-reverse permutation matrix, $\mathsf{P}^2=\mathsf{I}$ 

% $\mathsf{S_P}$ : decode matrix, $\mathsf{S_P} = \mathsf{SP}$

% $\mathbf{x_P}$, $\mathbf{y_P}$ : bit-reverse permutated vectors, $\mathbf{x_P} = \mathsf{P}\mathbf{x}$

%-------------------------------------------------------------------------------
% PAST ATTEMPTS:

% All full diagonal matrices with block size M have the same number of nonzero diagonals (N/2)/M=B .

% If feature maps and kernels are packed in a certain way, multiple SISO convolutions can be evaluated by applying localDFT to each, then evaluating elementwise multiplication. Here we describe this packing method. The kernel weights are slot encoded into plaintexts, and the feature maps are slot encoded then encrypted into ciphertexts.

% The exact way the feature maps and the kernels are padded does not matter as long as they are consistent for a layer. For example, padding can be applied to only the right and bottom sides of a kernel, such that in the final ${\iwidth}\times {\iwidth}$ space, the original kernel is located at the top-leftmost corner.

% An element of this padded input feature map of input channel $c_{in}$, at the $\ii$th row and ${\jj}$th column, will be denoted as $\mathbf{I^{c_{in}}}_{\ii, \jj}$ ($0 \le \ii, \jj < {\iwidth}$). An element at the $\ii$th row and $\jj$th column of the padded kernel, which generates values for the $c_{out}$th output feature map using the values of the $c_{in}$th input feature map, will be denoted as $\mathbf{K^{c_{out}, c_{in}}}_{\ii, \jj}$ ($0 \le \ii, \jj < {\iwidth}$).

% Now consider a ciphertext \ct{$\mathbf{x_0}$}, where padded feature maps corresponding to some input channels $\{c_0, c_1, ..., c_{B-1}\} \subseteq \{0, 1, ..., C_{in}-1\}$ are each flattened in row-major order, then permutated in bit-reversed order to fill the $B$ blocks of size $M$ inside $\mathbf{x_0} \in \mathbb{C}^{N/2}$.

% \[ (\mathbf{x_0})_{{Mb+\sigma_{\log_{2}M}({\iwidth}\cdot \ii + \jj)}} = \mathbf{{I}^{c_{b}}}_{{\iwidth}\cdot \ii + \jj} \]

% We then generate a plaintext \pt{$\mathbf{y_0}$}, where the kernel weights fill the $M$-sized blocks of $\mathbf{y_0} \in \mathbb{C}^{N/2}$ in a similar manner, but order is reversed during the flattening. The kernels correspond to the input channels chosen when packing $\mathbf{x_0}$, and some output channels $\{{c'}_0, {c'}_1, ..., {c'}_{B-1}\} \subseteq \{0, 1, ..., C_{out}-1\}$. For convenience, the bit reversal function is defined for negative values $-M<n<0$ as $\sigma_{\log_{2}M}(n)=\sigma_{\log_{2}M}(M+n)$.

% \[ (\mathbf{y_0})_{{Mb+\sigma_{\log_{2}M}(p - ({\iwidth}\cdot \ii + \jj))}} = \begin{cases}
%                                                                         \mathbf{{K}^{{c'}_b, c_{b}}}_{{\iwidth}\cdot \ii + \jj} & p - ({\iwidth}\cdot \ii + \jj) \ge 0\\
%                                                                         -j\mathbf{{K}^{{c'}_b, c_{b}}}_{{\iwidth}\cdot \ii + \jj} & p - ({\iwidth}\cdot \ii + \jj) < 0\\
% \end{cases} \]

% The $-j$ is multiplied when the indices are negative in order to cancel out the factor $j$ that gets multiplied when values wrap around during the $j$-cyclic convolution. $p$ is a fixed integer used to choose the position of the resulting feature map.

% Of course, the convolution in CNN is defined in reverse direction to the traditional convolution denoted as $\ast$ above. Thus for the above equation to be precise, each kernel must be flattened in reverse order when creating $\mathbf{{K}^{c_{b}}}$.

==> algo/sconv.tex <==
\begin{algorithm}
\caption{ Strided Conv2D in \name} \label{alg:lazy-SISO}
\textbf{Input} $ct_{i}$: input ciphertext, $W'$: filter plaintexts inversely rotated \\
\textbf{Output} $ct_{o}$: output ciphertext
\begin{algorithmic}[1] % <-- added '[1]' to control line numbering
    \STATE{// \textbf{MulFilter}\&\textbf{Sum$_{c_{i}}$}($ct_i,W$)}
    \FOR {$j_1= 0 ,\ldots,f-1 $}
        \FOR {$j_2= 0 ,\ldots,f-1 $}
            \STATE $ct'[j_1,j_2] \mathrel{+}=$ MulPt($ct_i, W'[j_1,j_2]$)
        \ENDFOR
    \ENDFOR
    % \STATE {\color{olive} // EndSubRoutine }
    \STATE{// \textbf{Slide$_1$}\&\textbf{Sum$_f$}($ct'$)}
    \FOR {$j_1= 0 ,\ldots,f-1 $}
        \FOR {$j_2= 0 ,\ldots,f-1 $}
            \STATE $r \leftarrow w_i(j_1- \frac{f-1}{2}) + (j_2 - \frac{f -1}{2})$
            \STATE $ct_{o} \mathrel{+}=$ CRot($ct'[j_1,j_2], -r$)
        \ENDFOR
    \ENDFOR
    % \STATE {\color{olive} // EndSubRoutine }
    \STATE \textbf{return} $ct_{o}$
\end{algorithmic}
\end{algorithm}

